Gluino Pair Production at the LHC: The Threshold

The next-to-leading order analysis of the cross section of hadronic gluino pair production close to threshold is presented. Within the framework of non-relativistic QCD a significant enhancement compared to fixed order perturbation theory is observed which originates from the characteristic remnant of the 1S peak below the nominal pair threshold. This enhancement is similar to the corresponding one for top production. However, as a consequence of the larger colour factor of the QCD potential the effect is significantly enhanced. The analysis includes all colour configurations of S-wave gluino pairs, i.e. singlet, symmetric and antisymmetric octet, decuplet and twenty-seven representation. Matching coefficients involving real and virtual radiation are separately evaluated for all colour and spin configurations and initial states. We concentrate on the case of gluino decay rates comparable to the gluino binding energy. The non-relativistic dynamics of the gluino pair is solved by calculating the Green's function in NLO. Numerical results for the Large Hadron Collider at sqrt(s)=14 TeV and 7 TeV are presented for various characteristic scenarios.

==> inclusions/main_ref.tex <==
%
% main_ref.tex -- generated by sortref-2.3.6  
% ((C) R. Harlander, http://www.robert-harlander.de/software/)
% on Thu Jul 28 17:43:02 CEST 2011
%

%1
\bibitem{Baer:2009dn}
  H.~Baer, V.~Barger, A.~Lessa and X.~Tata,
  JHEP {\bf 0909} (2009) 063
  [arXiv:0907.1922 [hep-ph]].
  %%CITATION = JHEPA,0909,063;%%

%2
\bibitem{Harrison:1982yi}
  P.~R.~Harrison and C.~H.~Llewellyn Smith,
  Nucl.\ Phys.\  B {\bf 213} (1983) 223
  [Erratum-ibid.\  B {\bf 223} (1983) 542].
  %%CITATION = NUPHA,B213,223;%%

%3
\bibitem{Haber:1984rc}
  H.~E.~Haber and G.~L.~Kane,
  Phys.\ Rept.\  {\bf 117}, 75 (1985).
  %%CITATION = PRPLC,117,75;%%

%4
\bibitem{Dawson:1983fw}
  S.~Dawson, E.~Eichten and C.~Quigg,
  Phys.\ Rev.\  D {\bf 31} (1985) 1581.
  %%CITATION = PHRVA,D31,1581;%%

%5
\bibitem{Beenakker:1996ch}
  W.~Beenakker, R.~H\"opker, M.~Spira and P.~M.~Zerwas,
  Nucl.\ Phys.\  B {\bf 492} (1997) 51
  [arXiv:hep-ph/9610490].
  %%CITATION = NUPHA,B492,51;%%

%6
\bibitem{Beenakker:1996ed}
  W.~Beenakker, R.~H\"opker and M.~Spira,
  arXiv:hep-ph/9611232.
  %%CITATION = HEP-PH/9611232;%%

%7
\bibitem{Beenakker:1997ut}
  W.~Beenakker, M.~Kr\"amer, T.~Plehn, M.~Spira and P.~M.~Zerwas,
  Nucl.\ Phys.\  B {\bf 515} (1998) 3
  [arXiv:hep-ph/9710451].
  %%CITATION = NUPHA,B515,3;%%

%8
\bibitem{Kulesza:2008jb}
  A.~Kulesza and L.~Motyka,
  Phys.\ Rev.\ Lett.\  {\bf 102} (2009) 111802
  [arXiv:0807.2405 [hep-ph]].
  %%CITATION = PRLTA,102,111802;%%

%9
\bibitem{Langenfeld:2009eg}
  U.~Langenfeld and S.~O.~Moch,
  Phys.\ Lett.\  B {\bf 675} (2009) 210
  [arXiv:0901.0802 [hep-ph]].
  %%CITATION = PHLTA,B675,210;%%

%10
\bibitem{Kulesza:2009kq}
  A.~Kulesza and L.~Motyka,
  Phys.\ Rev.\  D {\bf 80} (2009) 095004
  [arXiv:0905.4749 [hep-ph]].
  %%CITATION = PHRVA,D80,095004;%%

%11
\bibitem{Beenakker:2009ha}
  W.~Beenakker, S.~Brensing, M.~Kr\"amer, A.~Kulesza, E.~Laenen and I.~Niessen,
  JHEP {\bf 0912}, 041 (2009)
  [arXiv:0909.4418 [hep-ph]].
  %%CITATION = JHEPA,0912,041;%%

%12
\bibitem{Beenakker:2010nq}
  W.~Beenakker, S.~Brensing, M.~Kr\"amer, A.~Kulesza, E.~Laenen and I.~Niessen,
  JHEP {\bf 1008}, 098 (2010)
  [arXiv:1006.4771 [hep-ph]].
  %%CITATION = JHEPA,1008,098;%%

%13
\bibitem{Beneke:2010da}
  M.~Beneke, P.~Falgari, C.~Schwinn,
  Nucl.\ Phys.\  {\bf B842 } (2011) 414.
  [arXiv:1007.5414 [hep-ph]].

%14
\bibitem{Beenakker:2011fu}
  W.~Beenakker, S.~Brensing, M.~Kr\"amer, A.~Kulesza, E.~Laenen, L.~Motyka and I.~Niessen,
  Int.\ J.\ Mod.\ Phys.\  A {\bf 26} (2011) 2637
  [arXiv:1105.1110 [hep-ph]].
  %%CITATION = IMPAE,A26,2637;%%

%15
\bibitem{Kuhn:1992qw}
  J.~H.~K\"uhn and E.~Mirkes,
  Phys.\ Rev.\  D {\bf 48}, 179 (1993)
  [arXiv:hep-ph/9301204].
  %%CITATION = PHRVA,D48,179;%%

%16
\bibitem{Keung:1983wz}
  W.~Y.~Keung and A.~Khare,
  Phys.\ Rev.\  D {\bf 29}, 2657 (1984).
  %%CITATION = PHRVA,D29,2657;%%

%17
\bibitem{Kuhn:1983sc}
  J.~H.~K\"uhn and S.~Ono,
  Phys.\ Lett.\  B {\bf 142}, 436 (1984).
  %%CITATION = PHLTA,B142,436;%%

%18
\bibitem{Goldman:1984mj}
  J.~T.~Goldman and H.~Haber,
  Physica {\bf 15D}, 181 (1985).
  %%CITATION = PHYSA,15D,181;%%

%19
\bibitem{Kuhn:1987ty}
  J.~H.~K\"uhn and P.~M.~Zerwas,
  Phys.\ Rept.\  {\bf 167}, 321 (1988).
  %%CITATION = PRPLC,167,321;%%

%20
\bibitem{Kartvelishvili:1988tm}
  V.~G.~Kartvelishvili, A.~V.~Tkabladze and E.~G.~Chikovani,
  Z.\ Phys.\  C {\bf 43} (1989) 509.
  %%CITATION = ZEPYA,C43,509;%%

%21
\bibitem{Kartvelishvili:1989pp}
  V.~G.~Kartvelishvili, A.~V.~Tkabladze and E.~G.~Chikovani,
  Sov.\ J.\ Nucl.\ Phys.\  {\bf 51}, 546 (1990)
  [Yad.\ Fiz.\  {\bf 51}, 859 (1990)].
  %%CITATION = YAFIA,51,859;%%

%22
\bibitem{Chikovani:1996bk}
  E.~Chikovani, V.~Kartvelishvili, R.~Shanidze and G.~Shaw,
  Phys.\ Rev.\  D {\bf 53}, 6653 (1996)
  [arXiv:hep-ph/9602249].
  %%CITATION = PHRVA,D53,6653;%%

%23
\bibitem{Giudice:2004tc}
  G.~F.~Giudice and A.~Romanino,
  Nucl.\ Phys.\  B {\bf 699}, 65 (2004)
  [Erratum-ibid.\  B {\bf 706}, 65 (2005)]
  [arXiv:hep-ph/0406088].
  %%CITATION = NUPHA,B699,65;%%

%24
\bibitem{ArkaniHamed:2004fb}
  N.~Arkani-Hamed and S.~Dimopoulos,
  JHEP {\bf 0506}, 073 (2005)
  [arXiv:hep-th/0405159].
  %%CITATION = JHEPA,0506,073;%%

%25
\bibitem{Kilian:2004uj}
  W.~Kilian, T.~Plehn, P.~Richardson and E.~Schmidt,
  Eur.\ Phys.\ J.\  C {\bf 39}, 229 (2005)
  [arXiv:hep-ph/0408088].
  %%CITATION = EPHJA,C39,229;%%

%26
\bibitem{Cheung:2004ad}
  K.~Cheung and W.~Y.~Keung,
  Phys.\ Rev.\  D {\bf 71}, 015015 (2005)
  [arXiv:hep-ph/0408335].
  %%CITATION = PHRVA,D71,015015;%%

%27
\bibitem{Kauth:2009ud}
  M.~R.~Kauth, J.~H.~K\"uhn, P.~Marquard and M.~Steinhauser,
  Nucl.\ Phys.\  B {\bf 831} (2010) 285
  [arXiv:0910.2612 [hep-ph]].
  %%CITATION = NUPHA,B831,285;%%

%28
\bibitem{Hagiwara:2008df}
  K.~Hagiwara, Y.~Sumino and H.~Yokoya,
  Phys.\ Lett.\  B {\bf 666}, 71 (2008)
  [arXiv:0804.1014 [hep-ph]].
  %%CITATION = PHLTA,B666,71;%%

%29
\bibitem{Kiyo:2008bv}
  Y.~Kiyo, J.~H.~K\"uhn, S.~Moch, M.~Steinhauser and P.~Uwer,
  Eur.\ Phys.\ J.\  C {\bf 60} (2009) 375
  [arXiv:0812.0919 [hep-ph]].
  %%CITATION = EPHJA,C60,375;%%

%30
\bibitem{Hagiwara:2009hq}
  K.~Hagiwara and H.~Yokoya,
  JHEP {\bf 0910} (2009) 049
  [arXiv:0909.3204 [hep-ph]].
  %%CITATION = JHEPA,0910,049;%%

%31
\bibitem{Petrelli:1997ge}
  A.~Petrelli, M.~Cacciari, M.~Greco, F.~Maltoni and M.~L.~Mangano,
  Nucl.\ Phys.\  B {\bf 514} (1998) 245
  [arXiv:hep-ph/9707223].
  %%CITATION = NUPHA,B514,245;%%

%32
\bibitem{MacFarlane:1968vc}
  A.~J.~MacFarlane, A.~Sudbery and P.~H.~Weisz,
  Commun.\ Math.\ Phys.\  {\bf 11} (1968) 77.
  %%CITATION = CMPHA,11,77;%%

%33
\bibitem{Allanach:2002nj}
  B.~C.~Allanach {\it et al.},
in {\it Proc. of the APS/DPF/DPB Summer Study on the Future of Particle Physics (Snowmass 2001) } ed. N.~Graf,
  Eur.\ Phys.\ J.\  C {\bf 25} (2002) 113
  [arXiv:hep-ph/0202233].
  %%CITATION = EPHJA,C25,113;%%

%34
\bibitem{Djouadi:2002ze}
  A.~Djouadi, J.~L.~Kneur and G.~Moultaka,
  Comput.\ Phys.\ Commun.\  {\bf 176} (2007) 426
  [arXiv:hep-ph/0211331].
  %%CITATION = CPHCB,176,426;%%

%35
\bibitem{Muhlleitner:2003vg}
  M.~M\"uhlleitner, A.~Djouadi and Y.~Mambrini,
  Comput.\ Phys.\ Commun.\  {\bf 168}, 46 (2005)
  [arXiv:hep-ph/0311167].
  %%CITATION = CPHCB,168,46;%%

%36
\bibitem{Beneke:2009rj}
  M.~Beneke, P.~Falgari, C.~Schwinn,
  Nucl.\ Phys.\  {\bf B828 } (2010) 69.
  [arXiv:0907.1443 [hep-ph]].

%37
\bibitem{Bartels:1993ih}
  J.~Bartels,
  Z.\ Phys.\  C {\bf 60} (1993) 471.
  %%CITATION = ZEPYA,C60,471;%%

%38
\bibitem{Martin:2009iq}
  A.~D.~Martin, W.~J.~Stirling, R.~S.~Thorne and G.~Watt,
  arXiv:0901.0002 [hep-ph].
  %%CITATION = ARXIV:0901.0002;%%

%39
\bibitem{Chetyrkin:2000yt}
  K.~G.~Chetyrkin, J.~H.~K\"uhn, M.~Steinhauser,
  Comput.\ Phys.\ Commun.\  {\bf 133 } (2000)  43-65.
  [hep-ph/0004189].

%40
\bibitem{Harlander:2007wh}
  R.~V.~Harlander, L.~Mihaila and M.~Steinhauser,
  Phys.\ Rev.\  D {\bf 76} (2007) 055002
  [arXiv:0706.2953 [hep-ph]].
  %%CITATION = PHRVA,D76,055002;%%

%41
\bibitem{Fadin:1987wz}
  V.~S.~Fadin and V.~A.~Khoze,
  JETP Lett.\  {\bf 46}, 525 (1987)
  [Pisma Zh.\ Eksp.\ Teor.\ Fiz.\  {\bf 46}, 417 (1987)].
  %%CITATION = ZFPRA,46,417;%%

%42
\bibitem{Fadin:1988fn}
  V.~S.~Fadin and V.~A.~Khoze,
  Sov.\ J.\ Nucl.\ Phys.\  {\bf 48} (1988) 309
  [Yad.\ Fiz.\  {\bf 48} (1988) 487].
  %%CITATION = YAFIA,48,487;%%

%43
\bibitem{Fadin:1990wx}
  V.~S.~Fadin, V.~A.~Khoze and T.~Sj\"ostrand,
  Z.\ Phys.\  C {\bf 48}, 613 (1990).
  %%CITATION = ZEPYA,C48,613;%%

%44
\bibitem{Smirnov:2009fh}
  A.~V.~Smirnov, V.~A.~Smirnov and M.~Steinhauser,
  Phys.\ Rev.\ Lett.\  {\bf 104} (2010) 112002
  [arXiv:0911.4742 [hep-ph]].
  %%CITATION = PRLTA,104,112002;%%

%45
\bibitem{Smirnov:2008pn}
  A.~V.~Smirnov, V.~A.~Smirnov and M.~Steinhauser,
  Phys.\ Lett.\  B {\bf 668} (2008) 293
  [arXiv:0809.1927 [hep-ph]].
  %%CITATION = PHLTA,B668,293;%%

%46
\bibitem{Anzai:2009tm}
  C.~Anzai, Y.~Kiyo and Y.~Sumino,
  Phys.\ Rev.\ Lett.\  {\bf 104} (2010) 112003
  [arXiv:0911.4335 [hep-ph]].
  %%CITATION = PRLTA,104,112003;%%

%47
\bibitem{Anzai:2010td}
  C.~Anzai, Y.~Kiyo and Y.~Sumino,
  Nucl.\ Phys.\  B {\bf 838} (2010) 28
  [arXiv:1004.1562 [hep-ph]].
  %%CITATION = NUPHA,B838,28;%%

%48
\bibitem{Kniehl:2004rk}
  B.~A.~Kniehl, A.~A.~Penin, Y.~Schr\"oder, V.~A.~Smirnov and M.~Steinhauser,
  Phys.\ Lett.\  B {\bf 607} (2005) 96
  [arXiv:hep-ph/0412083].
  %%CITATION = PHLTA,B607,96;%%

%49
\bibitem{Beneke:1999qg}
  M.~Beneke, A.~Signer and V.~A.~Smirnov,
  Phys.\ Lett.\  B {\bf 454} (1999) 137
  [arXiv:hep-ph/9903260].
  %%CITATION = PHLTA,B454,137;%%

%50
\bibitem{Pineda:2006ri}
  A.~Pineda and A.~Signer,
  Nucl.\ Phys.\  B {\bf 762} (2007) 67
  [arXiv:hep-ph/0607239].
  %%CITATION = NUPHA,B762,67;%%

%51
\bibitem{Beneke:2005hg}
  M.~Beneke, Y.~Kiyo and K.~Schuller,
  Nucl.\ Phys.\  B {\bf 714}, 67 (2005)
  [arXiv:hep-ph/0501289].
  %%CITATION = NUPHA,B714,67;%%

%52
\bibitem{Hahn:2000kx}
  T.~Hahn,
  Comput.\ Phys.\ Commun.\  {\bf 140 } (2001)  418-431.
  [hep-ph/0012260].

%53
\bibitem{Hahn:2001rv}
  T.~Hahn, C.~Schappacher,
  Comput.\ Phys.\ Commun.\  {\bf 143 } (2002)  54-68.
  [hep-ph/0105349].

%54
\bibitem{Vermaseren:2000nd}
  J.~A.~M.~Vermaseren,
  [math-ph/0010025].

%55
\bibitem{Siegel:1979wq}
  W.~Siegel,
  Phys.\ Lett.\  B {\bf 84} (1979) 193.
  %%CITATION = PHLTA,B84,193;%%

%56
\bibitem{Martin:1993yx}
  S.~P.~Martin and M.~T.~Vaughn,
  Phys.\ Lett.\  B {\bf 318} (1993) 331
  [arXiv:hep-ph/9308222].
  %%CITATION = PHLTA,B318,331;%%

%57
\bibitem{Mihaila:2009bn}
  L.~Mihaila,
  Phys.\ Lett.\  B {\bf 681} (2009) 52
  [arXiv:0908.3403 [hep-ph]].
  %%CITATION = PHLTA,B681,52;%%

%58
\bibitem{Kuhn:1979bb}
  J.~H.~K\"uhn, J.~Kaplan and E.~G.~O.~Safiani,
  Nucl.\ Phys.\  B {\bf 157}, 125 (1979).
  %%CITATION = NUPHA,B157,125;%%

%59
\bibitem{Guberina:1980dc}
  B.~Guberina, J.~H.~K\"uhn, R.~D.~Peccei and R.~R\"uckl,
  Nucl.\ Phys.\  B {\bf 174}, 317 (1980).
  %%CITATION = NUPHA,B174,317;%%

%60
\bibitem{Kauth:2011phd}
  M.~R.~Kauth,
  PhD Thesis, KIT.

%61
\bibitem{Huber:2005yg}
  T.~Huber and D.~Maitre,
  Comput.\ Phys.\ Commun.\  {\bf 175} (2006) 122
  [arXiv:hep-ph/0507094].
  %%CITATION = CPHCB,175,122;%%

%62
\bibitem{'tHooft:1978xw}
  G.~'t Hooft and M.~J.~G.~Veltman,
  Nucl.\ Phys.\  B {\bf 153}, 365 (1979).
  %%CITATION = NUPHA,B153,365;%%


==> inclusions/realfunctions.tex <==
\begin{eqnarray}
\mathcal{F}_{gq}^{[1_s]}(z,r)&=&\Bigl[\,9r(r+1)^3z^4-(r-1)(r+1)^2z^3-2(r+1)(19r+35)z^2
\nonumber\\
&&\hspace{0.2cm}-32(r+1)z-64\Bigr]\frac{16z}{27\left[(r+1)z-2\right]^2\left[(r+1)z+2\right]^3}\ln(z)
\nonumber\\
&&\hspace{-0.3cm}+\Bigl[\,(r+1)^3(21r+5)z^4+2(r+1)^2(5r+9)z^3+4(r+1)(23r-29)z^2
\nonumber\\
&&\hspace{0.2cm}+200(r+1)z-224\Bigr]\frac{2z\left[5z(r+1)-8\right]\ln\left(1+2\frac{1-z}{z(r+1)}\right)}{243\left[(r+1)z-2\right]^2\left[(r+1)z+2\right]^3}
\nonumber\\
&&\hspace{-0.3cm}+\Bigl[\,(r+1)^3(57r+41)z^4+4(r+1)^2(81r^2+61r-36)z^3
\nonumber\\
&&\hspace{0.2cm}-4(r+1)(55r+71)z^2-16(r+1)(81r+133)z+256\Bigr]
\nonumber\\
&&\hspace{0.2cm}\times\frac{4(1-z)}{243(r+1)\left[z^2(r+1)^2-4\right]^2}\,,
\label{Fgq1}
\end{eqnarray}

\begin{eqnarray}
\mathcal{F}_{gq}^{[8_s]}(z,r)&=&\Bigl[\,9r(r+1)^3z^4-4(r-1)(r+1)^2z^3-4(r+1)(11r+26)z^2
\nonumber\\
&&\hspace{0.2cm}-40(r+1)z-80\Bigr]\frac{32z\ln(z)}{27\left[(r+1)z-2\right]^2\left[(r+1)z+2\right]^3}
\nonumber\\
&&\hspace{-0.3cm}+\Bigl[\,(r+1)^4(33r+28)z^5-4(r+1)^3(37r-14)z^4
\nonumber\\
&&\hspace{0.2cm}+4(r+1)^2(47r-175)z^3+8(r+1)(33r+163)z^2
\nonumber\\
&&\hspace{0.2cm}-16(86r+131)z+1120\Bigr]\frac{8z\ln\left(1+2\frac{1-z}{z(r+1)}\right)}{243\left[(r+1)z-2\right]^2\left[(r+1)z+2\right]^3}
\nonumber\\
&&\hspace{-0.3cm}+\Bigl[\,(r+1)^3(24r+19)z^4+(r+1)^2(81r^2+56r-45)z^3
\nonumber\\
&&\hspace{0.2cm}-4(r+1)(11r+16)z^2-4(r+1)(81r+191)z+80\Bigr]
\nonumber\\
&&\hspace{0.2cm}\times\frac{32(1-z)}{243(r+1)\left[z^2(r+1)^2-4\right]^2}
\,,
\nonumber\\
\label{Fgq8s}
\end{eqnarray}

\begin{eqnarray}
\mathcal{F}_{gq}^{[8_a]}(z,r)&=&\Bigl[\,9(r-1)^2(r+1)^4z^6+(r+1)^3(67r^2-186r+67)z^5
\nonumber\\
&&\hspace{0.2cm}-(r+1)^2(13r^3+207r^2-81r-67)z^4
\nonumber\\
&&\hspace{0.2cm}-2(r+1)^2(85r^2+100r-233)z^3-36(r+1)(5r^2-6r-3)z^2
\nonumber\\
&&\hspace{0.2cm}+72(7r^2\hspace{-0.05cm}+\hspace{-0.05cm}18r+3)z\hspace{-0.05cm}+\hspace{-0.05cm}576r\Bigr]\frac{32\ln(z)}{27(r+1)^2\left[(r+1)z\hspace{-0.05cm}-\hspace{-0.05cm}2\right]^2\left[(r+1)z\hspace{-0.05cm}+\hspace{-0.05cm}2\right]^3}
\nonumber\\
&&\hspace{-0.3cm}-\Bigl[\,(r+1)^4(3r^3+35r^2+13r+13)z^6
\nonumber\\
&&\hspace{0.2cm}-2(r+1)^3(35r^3-195r^2+353r-57)z^5
\nonumber\\
&&\hspace{0.2cm}-8(r+1)^2(5r^3+125r^2-189r+91)z^4
\nonumber\\
&&\hspace{0.2cm}+16(r+1)(15r^3+7r^2+25r+97)z^3
\nonumber\\
&&\hspace{0.2cm}+16(19r^3+11r^2-227r-91)z^2+32(r^2+82r+17)z-1024r\Bigr]
\nonumber\\
&&\hspace{0.2cm}\times\frac{4\ln\left(1+2\frac{1-z}{z(r+1)}\right)}{27(r+1)^2\left[(r+1)z-2\right]^2\left[(r+1)z+2\right]^3}
\nonumber\\
&&\hspace{-0.3cm}+\Bigl[\,(r-1)(r+1)^3(21r^2-38r+37)z^6
\nonumber\\
&&\hspace{0.2cm}+4(r+1)^2(35r^3-324r^2+327r-82)z^5
\nonumber\\
&&\hspace{0.2cm}-8(r+1)(6r^3+75r^2+136r-93)z^4
\nonumber\\
&&\hspace{0.2cm}-16(18r^4+25r^3-104r^2+61r+44)z^3
\nonumber\\
&&\hspace{0.2cm}-16(36r^3-23r^2-214r-115)z^2+384(3r^2+r-1)z+2304r\Bigr]
\nonumber\\
&&\hspace{0.2cm}\times\frac{8(1-z)}{27(r+1)^2z\left[z(r-1)+2\right]\left[z^2(r+1)^2-4\right]^2}\,,
\label{Fgq8a}
\end{eqnarray}

\begin{eqnarray}
\mathcal{F}_{gq}^{[10]}(z,r)&=&\Bigl[\,(r+1)(r^2-6r+1)z^2-(r-1)(r^2+10r+1)z
\nonumber\\
&&\hspace{0.2cm}-2(r^2-2r-11)\Bigr]\frac{320z^3\ln(z)}{27\left[(r+1)z-2\right]^2\left[(r+1)z+2\right]^3}
\nonumber\\
&&\hspace{-0.3cm}-\Bigl[\,(r+1)^5z^4+2(r+1)(3r^3+9r^2-23r+3)z^3
\nonumber\\
&&\hspace{0.2cm}+4(r^3-21r^2+3r-7)z^2-8(r^2+6r-11)z-64\Bigr]
\nonumber\\
&&\hspace{0.2cm}\times\frac{40z^2\ln\left(1+2\frac{1-z}{z(r+1)}\right)}{27\left[(r+1)z-2\right]^2\left[(r+1)z+2\right]^3}
\nonumber\\
&&\hspace{-0.3cm}+\Bigl[\,(r-1)(r+1)^3z^4+2(3r-1)(r^2\hspace{-0.05cm}-\hspace{-0.05cm}10r+5)z^3+4(3r^2\hspace{-0.05cm}-\hspace{-0.05cm}20r+9)z^2
\nonumber\\
&&\hspace{0.2cm}+8(5r-7)z+64\Bigr]\frac{80z(1-z)}{27\left[z(r-1)+2\right]\left[z^2(r+1)^2-4\right]^2}
\,,
\label{Fgq10}
\end{eqnarray}

\begin{eqnarray}
\mathcal{F}_{gq}^{[27_s]}(z,r)&=&\Bigl[\,r(r+1)z^2-(r-1)z-6\Bigr]\frac{16z^3(r+1)^2\ln(z)}{\left[(r+1)z-2\right]^2\left[(r+1)z+2\right]^3}
\nonumber\\
&&\hspace{-0.3cm}+\Bigl[\,(r+1)^4z^4-2(r+1)^2(3r-1)z^3-4(r+1)(r+5)z^2
\nonumber\\
&&\hspace{0.2cm}+8(r+1)z-32\Bigr]\frac{2z^2(r+1)\ln\left(1+2\frac{1-z}{z(r+1)}\right)}{\left[(r+1)z-2\right]^2\left[(r+1)z+2\right]^3}
\nonumber\\
&&\hspace{-0.3cm}+\Bigl[\,(r+1)z^2+2(2r+1)z+8\Bigr]\frac{4z(1-z)(r+1)}{\left[z(r+1)+2\right]\left[z^2(r+1)^2-4\right]}
\,,
\label{Fgq27}
\end{eqnarray}

\begin{eqnarray}
\mathcal{F}_{q\overline{q}}^{[1_s]}(z,r)&=&-\Bigl[\,18r^2(r^2+1)z^4+(81r^3\hspace{-0.05cm}-\hspace{-0.05cm}35r^2+27r\hspace{-0.05cm}-\hspace{-0.05cm}1)z^3+4(38r^2\hspace{-0.05cm}-\hspace{-0.05cm}13r+3)z^2
\nonumber\\
&&\hspace{0.6cm}+4(31r-5)z+36\Bigr]\frac{8z\left[(9r+1)z+8\right]\ln\left(1+2\frac{1-z}{z(r+1)}\right)}{729(1-z)^2(rz+1)^3}
\nonumber\\
&&\hspace{-0.0cm}+\Bigl[\,18r^2(r^2\hspace{-0.05cm}-\hspace{-0.05cm}1)z^4+(81r^3+37r^2\hspace{-0.05cm}-\hspace{-0.05cm}27r+1)z^3+4(29r^2+14r-3)z^2
\nonumber\\
&&\hspace{0.6cm}+2(35r+11)z+16\Bigr]\frac{16\left[(9r+1)z+8\right]}{729(r+1)(1-z)\left[(r-1)z+2\right](rz+1)^2}\,,
\label{Fqq1}
\end{eqnarray}

\begin{eqnarray}
\mathcal{F}_{q\overline{q}}^{[8_s]}(z,r)&=&-\Bigl[\,9r^2(9r+4)(r^2+1)z^5+(477r^4+18r^3+130r^2+36r-13)z^4
\nonumber\\
&&\hspace{0.6cm}+(1143r^3-44r^2+125r+52)z^3+2(668r^2-53r-1)z^2
\nonumber\\
&&\hspace{0.6cm}+2(391r-14)z+180\Bigr]\frac{32z\ln\left(1+2\frac{1-z}{z(r+1)}\right)}{729(1-z)^2(rz+1)^3}
\nonumber\\
&&\hspace{-0.0cm}+\Bigl[\,9r^2(r^2-1)(9r+4)z^5+(477r^4+342r^3-104r^2-36r+13)z^4
\nonumber\\
&&\hspace{0.6cm}+(981r^3+640r^2-73r-52)z^3+2(479r^2+253r+14)z^2
\nonumber\\
&&\hspace{0.6cm}+40(11r+3)z+80\Bigr]\frac{64}{729(r+1)(1-z)\left[(r-1)z+2\right](rz+1)^2}\,,
\label{Fqq8s}
\end{eqnarray}

\begin{eqnarray}
\mathcal{F}_{q\overline{q}}^{[8_a]}(z,r)&=&\Bigl[\,2r^3(9r^4+35r^3+41r^2-19r-2)z^6
\nonumber\\
&&\hspace{0.2cm}+(88r^6+264r^5+309r^4-146r^3-26r^2-2r+1)z^5
\nonumber\\
&&\hspace{0.2cm}+2r(104r^4+213r^3+271r^2-65r-3)z^4
\nonumber\\
&&\hspace{0.2cm}+(349r^4+386r^3+492r^2\hspace{-0.05cm}-\hspace{-0.05cm}58r\hspace{-0.05cm}-\hspace{-0.05cm}1)z^3+4(99r^3+52r^2+63r\hspace{-0.05cm}-\hspace{-0.05cm}2)z^2
\nonumber\\
&&\hspace{0.2cm}+2(125r^2+26r+29)z+64r\Bigr]\frac{\ln\left(1+2\frac{1-z}{z(r+1)}\right)}{12(r-1)^2(1-z)^2(rz+1)^3}
\nonumber\\
&&\hspace{-0.3cm}-\Bigl[\,2r^2(r-1)(9r^3+35r^2+35r-3)z^5
\nonumber\\
&&\hspace{0.2cm}+(88r^5+200r^4+129r^3-191r^2+15r-1)z^4
\nonumber\\
&&\hspace{0.2cm}+2(107r^4+125r^3+140r^2-91r+3)z^3
\nonumber\\
&&\hspace{0.2cm}+(329r^3+165r^2+215r-53)z^2+2(141r^2+54r+25)z
\nonumber\\
&&\hspace{0.2cm}+48(2r+1)\Bigr]\frac{1}{6(r-1)^2(1-z)\left[(r-1)z+2\right](rz+1)^2}\,,
\label{Fqq8a}
\end{eqnarray}

\begin{eqnarray}
\mathcal{F}_{q\overline{q}}^{[10]}(z,r)&=&\Bigl[\,8r^4z^4-(r^4-22r^3+6r-1)z^3-2(r^3-13r^2-5r+1)z^2
\nonumber\\
&&\hspace{0.2cm}+16rz+8\Bigr]\frac{160z^2\ln\left(1+2\frac{1-z}{z(r+1)}\right)}{81(1-z)^2(rz+1)^3}
\nonumber\\
&&\hspace{-0.3cm}-\Bigl[\,8r^2(r-1)z^3-(r^3-23r^2+9r+1)z^2-2(r^2-12r+3)z
\nonumber\\
&&\hspace{0.2cm}-2(r-7)\Bigr]\frac{320z^2}{81(1-z)\left[(r-1)z+2\right](rz+1)^2}\,,
\label{Fqq10}
\end{eqnarray}

\begin{eqnarray}
\mathcal{F}_{q\overline{q}}^{[27_s]}(z,r)&=&-\Bigl[\,2r^2(r^2+1)z^4+(3r^2+1)(3r-1)z^3+4(4r^2-r+1)z^2
\nonumber\\
&&\hspace{0.6cm}+4(3r-1)z+4\Bigr]\frac{8z^2(r+1)\ln\left(1+2\frac{1-z}{z(r+1)}\right)}{3(1-z)^2(rz+1)^3}
\nonumber\\
&&\hspace{-0.0cm}+\Bigl[\,2r^2(r-1)z^3+(9r^2-4r+1)z^2+4(3r-1)z+6\Bigr]
\nonumber\\
&&\hspace{0.6cm}\times\frac{16z^2(r+1)}{3(1-z)\left[(r-1)z+2\right](rz+1)^2}\,.
\label{Fqq27}
\end{eqnarray}

==> inclusions/tableSPS1.tex <==
\begin{tabular}{c||c|c|c|c|c|c|c}
benchmark&$m_{\tilde{g}}\,\left[\mbox{GeV}\right]$&$\overline{m}_{\tilde{q}}\,\left[\mbox{GeV}\right]$&$\Delta M\,\left[\mbox{GeV}\right]$&$2\Gamma_{\tilde{g}}\,\left[\mbox{GeV}\right]$&$\Gamma_{gg}\,\left[\mbox{GeV}\right]$&class&dominant decay
\\
point&&&&&&&channels
\\\hline\hline
(a)&$606.11$&$541.04$&$13.89$&$9.08$&$0.37$&$B$&$\tilde{g}\rightarrow\tilde{b}_{1}\overline{b},\tilde{b}^{*}_{1}b$
\\\hline
(b)&$493.05$&$443.19$&$12.04$&$6.28$&$0.34$&$B$&$\tilde{g}\rightarrow\tilde{c}_{2}\overline{c},\tilde{c}^{*}_{2}c,$
\\
&&&&&&&\hspace{0.8cm}$\tilde{u}_{2}\overline{u},\tilde{u}^{*}_{2}u$
\\\hline
(c)&$381.45$&$344.04$&$9.88$&$5.20$&$0.30$&$B$&$\tilde{g}\rightarrow\tilde{b}_{1}\overline{b},\tilde{b}^{*}_{1}b$
\\\hline
(d)&$717.12$&$637.39$&$15.75$&$12.00$&$0.40$&$B$&$\tilde{g}\rightarrow\tilde{b}_{1}\overline{b},\tilde{b}^{*}_{1}b$
\\\hline
(e)&$826.71$&$732.62$&$17.52$&$14.92$&$0.43$&$B$&$\tilde{g}\rightarrow\tilde{t}_{1}\overline{t},\tilde{t}^{*}_{1}t$
\\\hline
(f)&$935.18$&$826.94$&$19.22$&$17.84$&$0.46$&$B$&$\tilde{g}\rightarrow\tilde{b}_{1}\overline{b},\tilde{b}^{*}_{1}b$
\\\hline
(g)&$1042.60$&$920.35$&$20.87$&$20.70$&$0.48$&$B$&$\tilde{g}\rightarrow\tilde{t}_{1}\overline{t},\tilde{t}^{*}_{1}t$
\\\hline
(h)&$1149.42$&$1013.25$&$22.47$&$23.52$&$0.51$&$C$&$\tilde{g}\rightarrow\tilde{t}_{1}\overline{t},\tilde{t}^{*}_{1}t$
\\\hline
(i)&$936.42$&$831.88$&$19.24$&$16.38$&$0.46$&$B$&$\tilde{g}\rightarrow\tilde{b}_{1}\overline{b},\tilde{b}^{*}_{1}b$
\\\hline
(j)&$802.21$&$1462.40$&$17.13$&$0.0080$&$0.43$&$A$&$\tilde{g}\rightarrow\tilde{\chi}^{+}_{2}b\overline{t},\tilde{\chi}^{-}_{2}t\overline{b}$
\\\hline
(k)&$566.65$&$1219.50$&$13.21$&$0.0020$&$0.36$&$A$&$\tilde{g}\rightarrow\tilde{\chi}^{0}_{2}b\overline{b}$
\\\hline
(l)&$319.59$&$987.34$&$8.69$&$0.0002$&$0.28$&$A$&$\tilde{g}\rightarrow\tilde{\chi}^{+}_{1}d\overline{u},\tilde{\chi}^{-}_{1}u\overline{d},$
\\
&&&&&&&\hspace{0.5cm}$\tilde{\chi}^{+}_{1}s\overline{c},\tilde{\chi}^{-}_{1}c\overline{s}$
\\\hline
(m)&$1030.98$&$1710.01$&$20.69$&$0.022$&$0.48$&$A$&$\tilde{g}\rightarrow\tilde{\chi}^{+}_{2}b\overline{t},\tilde{\chi}^{-}_{2}t\overline{b}$
\\\hline
(n)&$1255.61$&$1959.83$&$24.04$&$0.044$&$0.53$&$A$&$\tilde{g}\rightarrow\tilde{\chi}^{+}_{2}b\overline{t},\tilde{\chi}^{-}_{2}t\overline{b}$
\\\hline
(o)&$933.03$&$819.58$&$19.19$&$19.26$&$0.46$&$C$&$\tilde{g}\rightarrow\tilde{t}_{1}\overline{t},\tilde{t}^{*}_{1}t$
\\\hline
(p)&$734.11$&$714.46$&$16.02$&$3.48$&$0.41$&$B$&$\tilde{g}\rightarrow\tilde{b}_{1}\overline{b},\tilde{b}^{*}_{1}b$
\\\hline
(q)&$719.66$&$618.86$&$15.79$&$22.92$&$0.40$&$C$&$\tilde{g}\rightarrow\tilde{t}_{1}\overline{t},\tilde{t}^{*}_{1}t$
\end{tabular}

==> inclusions/tableSPS2.tex <==
\begin{tabular}{c|c||c|c|c|c|c}
benchmark&SPS&$m_{0}\,\left[\mbox{GeV}\right]$&$m_{1/2}\,\left[\mbox{GeV}\right]$&$A_{0}\,\left[\mbox{GeV}\right]$&$\tan(\beta)$&$\mbox{sign}(\mu)$
\\
point&scenario&&&&&
\\\hline\hline
(a)&SPS1a-point&$100$&$250$&$-100$&$10$&$1$
\\\hline
(b)&SPS1a-slope1&$80$&$200$&$-80$&$10$&$1$
\\\hline
(c)&SPS1a-slope2&$60$&$150$&$-60$&$10$&$1$
\\\hline
(d)&SPS1a-slope3&$120$&$300$&$-120$&$10$&$1$
\\\hline
(e)&SPS1a-slope4&$140$&$350$&$-140$&$10$&$1$
\\\hline
(f)&SPS1a-slope5&$160$&$400$&$-160$&$10$&$1$
\\\hline
(g)&SPS1a-slope6&$180$&$450$&$-180$&$10$&$1$
\\\hline
(h)&SPS1a-slope7&$200$&$500$&$-200$&$10$&$1$
\\\hline
(i)&SPS1b-point&$200$&$400$&$0$&$30$&$1$
\\\hline
(j)&SPS2-point&$1450$&$300$&$0$&$10$&$1$
\\\hline
(k)&SPS2-slope1&$1250$&$200$&$0$&$10$&$1$
\\\hline
(l)&SPS2-slope2&$1050$&$100$&$0$&$10$&$1$
\\\hline
(m)&SPS2-slope3&$1650$&$400$&$0$&$10$&$1$
\\\hline
(n)&SPS2-slope4&$1850$&$500$&$0$&$10$&$1$
\\\hline
(o)&SPS3-point&$90$&$400$&$0$&$10$&$1$
\\\hline
(p)&SPS4-point&$400$&$300$&$0$&$50$&$1$
\\\hline
(q)&SPS5-point&$150$&$300$&$-1000$&$5$&$1$
\end{tabular}

==> inclusions/tableSPS3.tex <==
\begin{tabular}{c||c|c|c|c|c|c}
benchmark&$m_{\tilde{d}_{1}}\,\left[\mbox{GeV}\right]$&$m_{\tilde{d}_{2}}\,\left[\mbox{GeV}\right]$&$m_{\tilde{u}_{1}}\,\left[\mbox{GeV}\right]$&$m_{\tilde{u}_{2}}\,\left[\mbox{GeV}\right]$&$m_{\tilde{s}_{1}}\,\left[\mbox{GeV}\right]$&$m_{\tilde{s}_{2}}\,\left[\mbox{GeV}\right]$
\\
point&&&&&&
\\\hline\hline
(a)&$567.77$&$545.62$&$562.26$&$545.89$&$567.77$&$545.62$
\\\hline
(b)&$464.72$&$446.20$&$457.94$&$445.62$&$464.72$&$446.20$
\\\hline
(c)&$360.24$&$344.94$&$351.37$&$343.26$&$360.24$&$344.94$
\\\hline
(d)&$669.23$&$643.23$&$664.59$&$644.23$&$669.23$&$643.23$
\\\hline
(e)&$769.54$&$739.52$&$765.52$&$741.20$&$769.54$&$739.52$
\\\hline
(f)&$868.90$&$834.78$&$865.36$&$837.09$&$868.90$&$834.78$
\\\hline
(g)&$967.33$&$929.03$&$964.15$&$931.94$&$967.33$&$929.03$
\\\hline
(h)&$1065.22$&$1022.71$&$1062.35$&$1026.20$&$1065.23$&$1022.71$
\\\hline
(i)&$876.84$&$843.16$&$873.27$&$845.41$&$876.84$&$843.16$
\\\hline
(j)&$1556.70$&$1552.46$&$1554.76$&$1552.07$&$1556.70$&$1552.46$
\\\hline
(k)&$1300.76$&$1300.38$&$1298.41$&$1299.46$&$1300.76$&$1300.38$
\\\hline
(l)&$1055.59$&$1058.08$&$1052.65$&$1056.68$&$1055.59$&$1058.08$
\\\hline
(m)&$1817.49$&$1808.85$&$1815.83$&$1809.03$&$1817.49$&$1808.85$
\\\hline
(n)&$2080.64$&$2067.30$&$2079.20$&$2068.06$&$2080.64$&$2067.30$
\\\hline
(o)&$858.66$&$824.01$&$855.07$&$826.36$&$858.66$&$824.01$
\\\hline
(p)&$764.91$&$743.68$&$760.88$&$744.40$&$764.91$&$743.68$
\\\hline
(q)&$678.15$&$652.40$&$673.86$&$653.45$&$678.15$&$652.40$
\end{tabular}

==> inclusions/tableSPS4.tex <==
\begin{tabular}{c||c|c|c|c|c|c}
benchmark&$m_{\tilde{c}_{1}}\,\left[\mbox{GeV}\right]$&$m_{\tilde{c}_{2}}\,\left[\mbox{GeV}\right]$&$m_{\tilde{b}_{1}}\,\left[\mbox{GeV}\right]$&$m_{\tilde{b}_{2}}\,\left[\mbox{GeV}\right]$&$m_{\tilde{t}_{1}}\,\left[\mbox{GeV}\right]$&$m_{\tilde{t}_{2}}\,\left[\mbox{GeV}\right]$
\\
point&&&&&&
\\\hline\hline
(a)&$562.26$&$545.89$&$516.91$&$546.24$&$399.73$&$586.53$
\\\hline
(b)&$457.94$&$445.62$&$421.76$&$448.10$&$319.81$&$499.59$
\\\hline
(c)&$351.37$&$343.26$&$325.09$&$348.45$&$242.07$&$413.19$
\\\hline
(d)&$664.59$&$644.23$&$610.48$&$642.77$&$479.61$&$673.26$
\\\hline
(e)&$765.52$&$741.20$&$702.91$&$738.14$&$559.00$&$759.85$
\\\hline
(f)&$865.36$&$837.09$&$794.42$&$832.56$&$637.74$&$846.32$
\\\hline
(g)&$964.15$&$931.94$&$885.04$&$926.03$&$715.69$&$932.52$
\\\hline
(h)&$1062.35$&$1026.20$&$975.15$&$1018.98$&$793.11$&$1018.75$
\\\hline
(i)&$873.27$&$845.41$&$777.67$&$826.04$&$661.71$&$839.81$
\\\hline
(j)&$1554.76$&$1552.07$&$1298.73$&$1539.74$&$970.87$&$1307.45$
\\\hline
(k)&$1298.41$&$1299.46$&$1073.69$&$1289.26$&$789.69$&$1083.38$
\\\hline
(l)&$1052.65$&$1056.68$&$860.37$&$1048.57$&$622.94$&$870.89$
\\\hline
(m)&$1815.83$&$1809.03$&$1528.82$&$1794.54$&$1157.84$&$1536.48$
\\\hline
(n)&$2079.20$&$2068.06$&$1761.18$&$2051.40$&$1347.10$&$1767.83$
\\\hline
(o)&$855.07$&$826.36$&$792.13$&$822.99$&$649.29$&$842.40$
\\\hline
(p)&$760.88$&$744.40$&$617.79$&$685.28$&$546.52$&$696.19$
\\\hline
(q)&$673.86$&$653.45$&$561.85$&$650.48$&$248.72$&$649.57$
\end{tabular}
